What Have We Learned from OpenReview?

Anonymous peer review is used by the great majority of computer science conferences. OpenReview is such a platform that aims to promote openness in peer review process. The paper, (meta) reviews, rebuttals, and final decisions are all released to public. We collect 5,527 submissions and their 16,853 reviews from the OpenReview platform. We also collect these submissions' citation data from Google Scholar and their non-peer-reviewed versions from arXiv.org. By acquiring deep insights into these data, we have several interesting findings that could help understand the effectiveness of the public-accessible double-blind peer review process. Our results can potentially help writing a paper, reviewing it, and deciding on its acceptance.

==> cause.tex <==
\subsection{Causality Analysis}
\label{sec:casuse}
{\color{red}we have analyzed many interesting phenomena, and has gotten many factors that influence the score. These factors have a strong correlation between the score. 
In order to further explore the reasons that affect the score of the paper.
We designed a comparative experiment to analyze the existing causality.We put forward causality to analysis process which mainly includes four steps: modeling, intervention, evaluation, and inference. In the experiment, multivariate linear regression method is used for modeling and the model is trained by the ICLR2020 conference data set.The data set includes 1) the confidence of the reviewers,2) whether the paper is published on the arXiv website,3) the innovation of the paper,4) whether the motivation of the paper is clear,5) the adequacy of the experiment of the paper, 6) completeness of related workers,7) presentation quality, and 8) initial score of the reviewer.Besides,to ensure the fairness of the experiment, each factor is standardized, quantizing to [-1,1].
The independent variable is composed of seven factors in the data set: reviewer-level, novel, motivation, experiment, related work, presentation,  arXiv,and score of reviewers (private dependent variable).The intervention process controls the independent variable x in the modeling, which is represented by do(x).For example, analyzing the impact on the innovation of the paper over the score.

In this experiment,the usual practice of the intervention process is ignored control factor (e.g., ignore novelty factor), and the other 6 types of factors are used for multiple linear regression modeling.The evaluation stage compares the Mean Square Error(MSE) obtained by the experimental group and the control group.In the inference stage, based on the comparison results in the evaluation stage, make causal inferences.
In this article,we set up seven experimental groups and a control group.The experimental group was compared with the control group.To reduce the error caused by the randomness of the experimental results.According to the law of large numbers, the probability of the result of multiple experiments is closer to the expected value.
This experiment is carried out 1000 times,and the result of the experiment is the mean value of the mean square error shown in table {\ref{cause1}
% {\color{red}{To further explore whether the factors that have correlation results are the reasons for the difference in scores. we conduct experiments to analyze the causal relationship. The factors designed in the experiment include the level of reviewers, whether to publish on arXiv, novel, motivation, experiment, related work, and presentation in sentiment analysis.In order to be able to distinguish the impact of various factors on the score, a comparative experiment was conducted. The control group received multiple linear regression training for multiple factors.When the external conditions are completely consistent, the experimental group intervenes in one of the factors. Generally speaking, the real cause is limited and may produce the desired result. But indirect reasons may produce random results.To eliminate this randomness, use the principle of the law of large numbers. The experiments were carried out 1000 epoch.The result is as shown table {\ref{cause1}}.
\vspace{-0.2in}
\begin{table}[H]
    \centering
    \caption{
Comparative Experiment Results}
    \label{cause1}
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    do(x)&reivewer-level&novel&motivation&experiment&related work&presentation&arXiv\\
    \hline
   ConMSE& 0.24& 0.24& 0.24& 0.24& 0.24& 0.24& 0.24\\
   \hline
   ExpMSE& 0.84& 0.77& 0.34& 0.86& 0.33& 0.34& 0.29\\
    \hline
    \end{tabular}
\end{table}
\vspace{-0.2in}
It can be seen from the table that when the various factors are intervened, the MSE of the experimental group became larger.At the same time, the three factors, reviewer-level, experiment and novel changed MSE even more. Comparing these three factors can more powerfully explain the reasons for the changes in scores.

% Rebuttal is an important part of the opening review process.Marginal articles can improve the probability of inclusion of articles through the Rebuttal process.It is generally agreed that Rebuttal is the cause of the change in opening review scores. We conduct comparative experiments to illustrate this phenomenon. The experimental data is the ICLR2020 data set. The control group remained unchanged, and the independent variables are still seven factors.The dependent variable is the initial rating of the reviewer.
% The independent variable of the experimental group increased the Rebuttal factor. The dependent variable is the final score of the reviewer. This experiment is carried out 3000 times, and compare the average of the experimental results shown in table {\ref{rebuttal}}



% % From the table,different experiments of the situation are compared to find the change of the mean square error.The experimental results show that the MSE generated by the training increases by interfering with a certain result, showing that there is a certain causal relationship.
% % As is known,rebuttal is also an important factor affecting the score. We conducted comparative experiments to prove the conclusions we already know. Experimental data is ICLR2020 data. The label of the control group is the score before rebuttal.The experimental group is the label is the final score. Many experiments have been carried out, and the experimental results are shown in the table {\ref{rebuttal}}.
% \begin{table}[H]
%     \centering
%     \caption{Rebuttal Comparative experiment results}
%     \label{rebuttal}
%     \setlength{\tabcolsep}{4.2mm}{
%     \begin{tabular}{c|c|c|c|c|c|c}
%     %\caption{T test calculate p value}
%     \hline
%     EPOCH & 500 & 1000& 1500& 2000& 2500& 3000\\
%     \hline
% ControlMSE & 0.83 & 0.24 & 0.31 & 0.44 & 0.30 & 0.28\\
%  \hline
% ExperimentMSE & 0.24 & 0.21 & 0.33 & 0.31 & 0.18 & 0.25\\
%     \hline
%     \end{tabular}}
% \end{table}
% we observed from the table that after adding the Rebuttal factor, the mean square error of the experimental group becomes smaller. To some extent, it can be said that the Rebuttal stage has a positive impact on the score.
% The experimental results show that rebuttal can be found to have an effect on the final score.
}}

==> chinese.tex <==
\subsection{Are Chinese Reviewers More Tough?}
\label{sec:review:chinese}
\begin{CJK}{UTF8}{gbsn}
  在ICLR2020中，华人作者投稿数量大增，因此推断reviewer中中国人的数量也会占据相当一部分比例。因此讨论中国人是否会倾向于打分较高/较低。
1. 如何在review中区分中国人
首先，我们收集了中国大学生所写的英语作文200+段，中国托福范文书中的作文500+段，分别构建了两个标准语法向量，该语法向量为1*10，其中描述了常用的语法词性noun，proper noun， coordinating,conjunction，modal，determiner，conjunction,\par
preposition/subordinating ，adjective，adverb，verb等的使用频率。接下来，将2020年全部paper的review共7766条分别构建语法向量，分别计算每一条review的语法向量与标准语法向量的距离，距离越小则认为他的语法风格更像是中国人。
2. 中国人是否打分偏高/偏低
我们按照语法向量的距离将这些review进行排序，计算距离最小的前x条review打分的平均值，与全部review打分平均值进行比较，并且计算一定区间内打分的平均值来更好的观察趋势，得到以下两图:
\begin{figure}[htbp]
    \subfloat[tf]{\includegraphics[width = 2in]{fig/tf.eps}\label{fig:tf}}\ \
    \subfloat[uv]{\includegraphics[width = 2in]{fig/uv.eps}\label{fig:uv}}\ \
    \caption{tf 与 uv 图}
    \label{fig:vpt}
    \vspace{-0.1in}
\end{figure}
从图中可以看出，在2020年
\end{CJK}

